User Personas Improve Social Sustainability by Encouraging Software Developers to Deprioritize Antisocial Features

Sustainable software development involves creating software in a manner that meets present goals without undermining our ability to meet future goals. In a software engineering context, sustainability has at least four dimensions: ecological, economic, social, and technical. No interventions for improving social sustainability in software engineering have been tested in rigorous lab-based experiments, and little evidence-based guidance is available. The purpose of this study is to evaluate the effectiveness of two interventions-stakeholder maps and persona models-for improving social sustainability through software feature prioritization. We conducted a randomized controlled factorial experiment with 79 undergraduate computer science students. Participants were randomly assigned to one of four groups and asked to prioritize a backlog of prosocial, neutral, and antisocial user stories for a shopping mall's digital screen display and facial recognition software. Participants received either persona models, a stakeholder map, both, or neither. We compared the differences in prioritization levels assigned to prosocial and antisocial user stories using Cumulative Link Mixed Model regression. Participants who received persona models gave significantly lower priorities to antisocial user stories but no significant difference was evident for prosocial user stories. The effects of the stakeholder map were not significant. The interaction effects were not significant. Providing aspiring software professionals with well-crafted persona models causes them to de-prioritize antisocial software features. The impact of persona modelling on sustainable software development therefore warrants further study with more experience professionals. Moreover, the novel methodological strategy of assessing social sustainability behavior through backlog prioritization appears feasible in lab-based settings.

==> TODO.tex <==

- finish the data extraction spreadsheet and upload it to Figshare. Make sure the address to the replication package in the paper is still correct. - SEAN (DEC 19) Done
- update the jupyter notebook, add it to figshare and refresh figs - SEAN (DEC 19) 
- the full citations of the core result set in the paper - ERIN (DEC 19) - Done
- update all the numbers on overleaf (e.g. numbers of primary studies) including table II - ERIN (DEC 19) - mostly done, just waiting on a couple of new figs
- a revision (or removal) of the diagram - PAUL DONE
- a detailed characterization of stratification as outlined in response 2 - PAUL DONE
- fix all minor errors mentioned by reviews - BIMPE (DEC 19)
- Look at the one paper that could be added to the synthesis and see how to fit it in somewhere: How Could We Have Known? Anticipating Sustainability Effects of a Software Product - BIMPE (DEC 19)


Summary of How Could We Have Known? Paper
The authors conducted a case study to show how the Sustainability Awareness Framework (SusAF) can be applied to identify the potential sustainability effects of an IT company’s (software) product.

The paper fits into proposition 1, since the aim of the case study was to identify the sustainability effects of the company’s financial management software. Before the case study, the company recognized only three sustainability effects that their financial management software might have, but with the Sustainability Awareness Framework (SusAF), 28 direct (first-order) effects, approx 100 enabling (second-order) effects and 23 structural (third-order) effects and several chains of effects, which were finally grouped into six high-level categories were identified. 

The authors also cited examples of how the different effects relates to sustainability.



==> tables/analysis.tex <==
# Load your data
# Replace 'path_to_your_data.csv' with the actual path to your CSV file
data <- read.csv('~/Downloads/Sustainability Experiment/firstentrydata.csv')

# Filter for prosocial stories
prosocial_data <- subset(data, story_type == "social")

# Create binary indicators
prosocial_data$persona_only <- as.numeric(prosocial_data$persona == 1 & prosocial_data$stakeholdermap == 0)
prosocial_data$stakeholdermap_only <- as.numeric(prosocial_data$persona == 0 & prosocial_data$stakeholdermap == 1)
prosocial_data$both <- as.numeric(prosocial_data$persona == 1 & prosocial_data$stakeholdermap == 1)

# Convert 'Prioritization_Level' to a factor
prosocial_data$Prioritization_Level <- factor(prosocial_data$Prioritization_Level)

# Fit the cumulative link mixed model
model <- clmm(Prioritization_Level ~ persona_only + stakeholdermap_only + both + (1 | Participant.ID), 
              data = prosocial_data, 
              link = "logit")

# Summary of the model
summary(model)

# Calculating Odds Ratios
odds_ratios <- exp(coef(model))

# Print the Odds Ratios
print(odds_ratios)
